PRISE: LLM-Style Sequence Compression for Learning Temporal Action Abstractions in Control

Temporal action abstractions, along with belief state representations, are a powerful knowledge sharing mechanism for sequential decision making. In this work, we propose a novel view that treats inducing temporal action abstractions as a sequence compression problem. To do so, we bring a subtle but critical component of LLM training pipelines -- input tokenization via byte pair encoding (BPE) -- to the seemingly distant task of learning skills of variable time span in continuous control domains. We introduce an approach called Primitive Sequence Encoding (PRISE) that combines continuous action quantization with BPE to learn powerful action abstractions. We empirically show that high-level skills discovered by PRISE from a multitask set of robotic manipulation demonstrations significantly boost the performance of both multitask imitation learning as well as few-shot imitation learning on unseen tasks. Our code is released at https://github.com/FrankZheng2022/PRISE.

==> app_pretraining_dataset_size.tex <==
\section{Impact of pretraining dataset size}
In the main experiments, we have primarily focused on examining the effects of \algo pretrained skill tokens for efficient downstream few-shot imitation learning under a fixed dataset. 
To further study how much data is needed to learn a good temporal action abstraction in \algo, we conduct a set of additional experiments on LIBERO. 
Instead of using the entire LIBERO-90 dataset, where each task includes 50 human demonstration trajectories, we now sample $N$ trajectories per task, with $N\in \{10,20,30,40\}$. We then evaluate the downstream performance of the \algo skill token, and the result is shown in Figure~\ref{fig:dataset_size}.
\begin{figure*}[!h]
\centering
\includegraphics[width=0.35\textwidth]{figures/libero_datasetsize.png}
\caption{Downstream performance of \algo under different pretraining dataset size}
\label{fig:dataset_size}
\end{figure*}
From the Figure, it is evident that the performance of \algo monotonically gets better as the number of pretraining trajectories per task increases. Notably, the performance of \algo is good with up to 40 trajectories per task but drops significantly with fewer than 30 trajectories per task. It would be interesting for future work to further scale up the existing LIBERO-90 dataset so that \algo may further benefit from an even larger pretraining dataset. But this should be beyond the scope of the current work.




==> shortcuts.tex <==
% last update: 2023-09-12
% created by Ching-An Cheng

% PACKAGES
% math
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage[inline]{enumitem}
%\usepackage{mathrsfs} 
%\usepackage{wrapfig}
\usepackage{thmtools,thm-restate}
% algorithms
\usepackage{algorithm}
\usepackage{algorithmic}
% misc
\usepackage{hyperref}
\usepackage{url}
\usepackage[capitalise,noabbrev]{cleveref}
\usepackage{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage{graphicx}
\usepackage{makecell}
\usepackage{comment}

%\usepackage[page]{appendix}
%\renewcommand{\appendixpagename}{\centering Appendix}

%\usepackage[numbers]{natbib}
% \usepackage[square,sort,comma,numbers]{natbib}



% EDITS
\newcommand{\todo}[1]{{\leavevmode\color{red}TODO: #1}}
\newcommand{\rev}[1]{{\leavevmode\color{blue}#1}}
\newcommand{\note}[1]{{\leavevmode\color{Green}Note: #1}}

% SHORTCUTS
% theorem setting
\renewcommand\qedsymbol{$\blacksquare$}

\theoremstyle{plain}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
\newtheorem{assumption}{Assumption}[section]

\newenvironment{proofsketch}{\textit{Proof sketch:}}{\qed \par}


% colors
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\pink}[1]{\textcolor{magenta}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}

% fonts
\def\AA{\mathcal{A}}\def\BB{\mathcal{B}}\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}\def\EE{\mathcal{E}}\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}\def\HH{\mathcal{H}}\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}\def\KK{\mathcal{K}}\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}\def\NN{\mathcal{N}}\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}\def\QQ{\mathcal{Q}}\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}\def\TT{\mathcal{T}}\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}\def\WW{\mathcal{W}}\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}\def\ZZ{\mathcal{Z}}

\def\Ab{\mathbf{A}}\def\Bb{\mathbf{B}}\def\Cb{\mathbf{C}}
\def\Db{\mathbf{D}}\def\Eb{\mathbf{E}}\def\Fb{\mathbf{F}}
\def\Gb{\mathbf{G}}\def\Hb{\mathbf{H}}\def\Ib{\mathbf{I}}
\def\Jb{\mathbf{J}}\def\Kb{\mathbf{K}}\def\Lb{\mathbf{L}}
\def\Mb{\mathbf{M}}\def\Nb{\mathbf{N}}\def\Ob{\mathbf{O}}
\def\Pb{\mathbf{P}}\def\Qb{\mathbf{Q}}\def\Rb{\mathbf{R}}
\def\Sb{\mathbf{S}}\def\Tb{\mathbf{T}}\def\Ub{\mathbf{U}}
\def\Vb{\mathbf{V}}\def\Wb{\mathbf{W}}\def\Xb{\mathbf{X}}
\def\Yb{\mathbf{Y}}\def\Zb{\mathbf{Z}}

% \sb could have conflict with \url package.
\def\ab{\mathbf{a}}\def\bb{\mathbf{b}}\def\cb{\mathbf{c}}
\def\db{\mathbf{d}}\def\eb{\mathbf{e}}\def\fb{\mathbf{f}}
\def\gb{\mathbf{g}}\def\hb{\mathbf{h}}\def\ib{\mathbf{i}}
\def\jb{\mathbf{j}}\def\kb{\mathbf{k}}\def\lb{\mathbf{l}}
\def\mb{\mathbf{m}}\def\nb{\mathbf{n}}\def\ob{\mathbf{o}}
\def\pb{\mathbf{p}}\def\qb{\mathbf{q}}\def\rb{\mathbf{r}}
\def\sb{\mathbf{s}}\def\tb{\mathbf{t}}\def\ub{\mathbf{u}}
\def\vb{\mathbf{v}}\def\wb{\mathbf{w}}\def\xb{\mathbf{x}}
\def\yb{\mathbf{y}}\def\zb{\mathbf{z}}

\def\Abb{\mathbb{A}}\def\Bbb{\mathbb{B}}\def\Cbb{\mathbb{C}}
\def\Dbb{\mathbb{D}}\def\Ebb{\mathbb{E}}\def\Fbb{\mathbb{F}}
\def\Gbb{\mathbb{G}}\def\Hbb{\mathbb{H}}\def\Ibb{\mathbb{I}}
\def\Jbb{\mathbb{J}}\def\Kbb{\mathbb{K}}\def\Lbb{\mathbb{L}}
\def\Mbb{\mathbb{M}}\def\Nbb{\mathbb{N}}\def\Obb{\mathbb{O}}
\def\Pbb{\mathbb{P}}\def\Qbb{\mathbb{Q}}\def\Rbb{\mathbb{R}}
\def\Sbb{\mathbb{S}}\def\Tbb{\mathbb{T}}\def\Ubb{\mathbb{U}}
\def\Vbb{\mathbb{V}}\def\Wbb{\mathbb{W}}\def\Xbb{\mathbb{X}}
\def\Ybb{\mathbb{Y}}\def\Zbb{\mathbb{Z}}

\def\Af{\mathfrak{A}}\def\Bf{\mathfrak{B}}\def\Cf{\mathfrak{C}}
\def\Df{\mathfrak{D}}\def\Ef{\mathfrak{E}}\def\Ff{\mathfrak{F}}
\def\Gf{\mathfrak{G}}\def\Hf{\mathfrak{H}}\def\If{\mathfrak{I}}
\def\Jf{\mathfrak{J}}\def\Kf{\mathfrak{K}}\def\Lf{\mathfrak{L}}
\def\Mf{\mathfrak{M}}\def\Nf{\mathfrak{N}}\def\Of{\mathfrak{O}}
\def\Pf{\mathfrak{P}}\def\Qf{\mathfrak{Q}}\def\Rf{\mathfrak{R}}
\def\Sf{\mathfrak{S}}\def\Tf{\mathfrak{T}}\def\Uf{\mathfrak{U}}
\def\Vf{\mathfrak{V}}\def\Wf{\mathfrak{W}}\def\Xf{\mathfrak{X}}
\def\Yf{\mathfrak{Y}}\def\Zf{\mathfrak{Z}}

\def\Av{\boldsymbol{A}}\def\Bv{\boldsymbol{B}}\def\Cv{\boldsymbol{C}}
\def\Dv{\boldsymbol{D}}\def\Ev{\boldsymbol{E}}\def\Fv{\boldsymbol{F}}
\def\Gv{\boldsymbol{G}}\def\Hv{\boldsymbol{H}}\def\Iv{\boldsymbol{I}}
\def\Jv{\boldsymbol{J}}\def\Kv{\boldsymbol{K}}\def\Lv{\boldsymbol{L}}
\def\Mv{\boldsymbol{M}}\def\Nv{\boldsymbol{N}}\def\Ov{\boldsymbol{O}}
\def\Pv{\boldsymbol{P}}\def\Qv{\boldsymbol{Q}}\def\Rv{\boldsymbol{R}}
\def\Sv{\boldsymbol{S}}\def\Tv{\boldsymbol{T}}\def\Uv{\boldsymbol{U}}
\def\Vv{\boldsymbol{V}}\def\Wv{\boldsymbol{W}}\def\Xv{\boldsymbol{X}}
\def\Yv{\boldsymbol{Y}}\def\Zv{\boldsymbol{Z}}

\def\av{\boldsymbol{a}}\def\bv{\boldsymbol{b}}\def\cv{\boldsymbol{c}}
\def\dv{\boldsymbol{d}}\def\ev{\boldsymbol{e}}\def\fv{\boldsymbol{f}}
\def\gv{\boldsymbol{g}}\def\hv{\boldsymbol{h}}\def\iv{\boldsymbol{i}}
\def\jv{\boldsymbol{j}}\def\kv{\boldsymbol{k}}\def\lv{\boldsymbol{l}}
\def\mv{\boldsymbol{m}}\def\nv{\boldsymbol{n}}\def\ov{\boldsymbol{o}}
\def\pv{\boldsymbol{p}}\def\qv{\boldsymbol{q}}\def\rv{\boldsymbol{r}}
\def\sv{\boldsymbol{s}}\def\tv{\boldsymbol{t}}\def\uv{\boldsymbol{u}}
\def\vv{\boldsymbol{v}}\def\wv{\boldsymbol{w}}\def\xv{\boldsymbol{x}}
\def\yv{\boldsymbol{y}}\def\zv{\boldsymbol{z}}

\def\Att{\mathtt{A}}\def\Btt{\mathtt{B}}\def\Ctt{\mathtt{C}}
\def\Dtt{\mathtt{D}}\def\Ett{\mathtt{E}}\def\Ftt{\mathtt{F}}
\def\Gtt{\mathtt{G}}\def\Htt{\mathtt{H}}\def\Itt{\mathtt{I}}
\def\Jtt{\mathtt{J}}\def\Ktt{\mathtt{K}}\def\Ltt{\mathtt{L}}
\def\Mtt{\mathtt{M}}\def\Ntt{\mathtt{N}}\def\Ott{\mathtt{O}}
\def\Ptt{\mathtt{P}}\def\Qtt{\mathtt{Q}}\def\Rtt{\mathtt{R}}
\def\Stt{\mathtt{S}}\def\Ttt{\mathtt{T}}\def\Utt{\mathtt{U}}
\def\Vtt{\mathtt{V}}\def\Wtt{\mathtt{W}}\def\Xtt{\mathtt{X}}
\def\Ytt{\mathtt{Y}}\def\Ztt{\mathtt{Z}}

\def\att{\mathtt{a}}\def\btt{\mathtt{b}}\def\ctt{\mathtt{c}}
\def\dtt{\mathtt{d}}\def\ett{\mathtt{e}}\def\ftt{\mathtt{f}}
\def\gtt{\mathtt{g}}\def\htt{\mathtt{h}}\def\itt{\mathtt{i}}
\def\jtt{\mathtt{j}}\def\ktt{\mathtt{k}}\def\ltt{\mathtt{l}}
\def\mtt{\mathtt{m}}\def\ntt{\mathtt{n}}\def\ott{\mathtt{o}}
\def\ptt{\mathtt{p}}\def\qtt{\mathtt{q}}\def\rtt{\mathtt{r}}
\def\stt{\mathtt{s}}\def\ttt{\mathtt{t}}\def\utt{\mathtt{u}}
\def\vtt{\mathtt{v}}\def\wtt{\mathtt{w}}\def\xtt{\mathtt{x}}
\def\ytt{\mathtt{y}}\def\ztt{\mathtt{z}}

\def\Asf{\mathsf{A}}\def\Bsf{\mathsf{B}}\def\Csf{\mathsf{C}}
\def\Dsf{\mathsf{D}}\def\Esf{\mathsf{E}}\def\Fsf{\mathsf{F}}
\def\Gsf{\mathsf{G}}\def\Hsf{\mathsf{H}}\def\Isf{\mathsf{I}}
\def\Jsf{\mathsf{J}}\def\Ksf{\mathsf{K}}\def\Lsf{\mathsf{L}}
\def\Msf{\mathsf{M}}\def\Nsf{\mathsf{N}}\def\Osf{\mathsf{O}}
\def\Psf{\mathsf{P}}\def\Qsf{\mathsf{Q}}\def\Rsf{\mathsf{R}}
\def\Ssf{\mathsf{S}}\def\Tsf{\mathsf{T}}\def\Usf{\mathsf{U}}
\def\Vsf{\mathsf{V}}\def\Wsf{\mathsf{W}}\def\Xsf{\mathsf{X}}
\def\Ysf{\mathsf{Y}}\def\Zsf{\mathsf{Z}}

\def\asf{\mathsf{a}}\def\bsf{\mathsf{b}}\def\csf{\mathsf{c}}
\def\dsf{\mathsf{d}}\def\esf{\mathsf{e}}\def\fsf{\mathsf{f}}
\def\gsf{\mathsf{g}}\def\hsf{\mathsf{h}}\def\isf{\mathsf{i}}
\def\jsf{\mathsf{j}}\def\ksf{\mathsf{k}}\def\lsf{\mathsf{l}}
\def\msf{\mathsf{m}}\def\nsf{\mathsf{n}}\def\osf{\mathsf{o}}
\def\psf{\mathsf{p}}\def\qsf{\mathsf{q}}\def\rsf{\mathsf{r}}
\def\ssf{\mathsf{s}}\def\tsf{\mathsf{t}}\def\usf{\mathsf{u}}
\def\vsf{\mathsf{v}}\def\wsf{\mathsf{w}}\def\xsf{\mathsf{x}}
\def\ysf{\mathsf{y}}\def\zsf{\mathsf{z}}



% math
\def\R{\Rbb}\def\Q{\Qbb}\def\Z{\Zbb}\def\N{\Nbb}\def\C{\Cbb}
\def\one{{\mathbbm1}}
\def\oneb{{\mathbf1}}
\def\zero{{\mathbbm0}}
\def\zerob{{\mathbf0}}
\def\GP{\GG\PP}
\def\K{\mathcal{K}}
\def\der{\mathrm{d}}
\def\zinf{[0, \infty) }
\def\afsystem{\dot{x}  =f(x) + g(x)u}
\def\const{\mathrm{const.}}
\def\diag{\mathrm{diag}}
\def\bdiag{\mathrm{blkdiag}}
\def\mvec{\mathrm{vec}}
\def\t{\top}
\def\*{\star}
%\def\mhef{\text{--}}
\DeclareMathSymbol{\mhef}{\mathord}{operators}{`\-}


\newcommand{\norm}[1]{ \| #1 \|  }
\newcommand{\abs}[1]{ \left| #1 \right|  }
\newcommand{\tr}[1]{ \mathrm{tr}\left( #1\right)}
\newcommand{\lr}[2]{ \left\langle #1, #2 \right\rangle}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% online learning
\def\regret{\textrm{Regret}}

% statistics
\newcommand{\KL}[2]{D_{KL}(#1, #2)} %\newcommand{\KL}[2]{KL[#1 || #2  ]}
\newcommand{\TV}[2]{D_{TV}(#1, #2)}
\newcommand{\HE}[2]{D_{H}(#1, #2)}
\newcommand{\WA}[2]{D_{W}(#1, #2)}
\newcommand{\FD}[2]{D_{f}(#1, #2)}
\newcommand{\E}{\Ebb}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}


% % Below is the code for optionally collecting all the proofs at the end
% % source: https://tex.stackexchange.com/questions/33229/how-to-place-all-proofs-automatically-in-appendix
% \usepackage{etex,etoolbox}
% %\usepackage{amsthm,amssymb}
% %\usepackage{thmtools}
% \usepackage{environ}

% \makeatletter
% \providecommand{\@fourthoffour}[4]{#4}
% % We define an addition for the theorem-like environments; when
% % \newtheorem{thm}{Theorem} is declared, the macro \thm expands
% % to {...}{...}{...}{Theorem} and with \@fourthoffour we access
% % to it; then we make available \@currentlabel (the theorem number)
% % also outside the environment.
% \newcommand\fixstatement[2][\proofname\space of]{%
% 	\ifcsname thmt@original@#2\endcsname
% 	% the theorem has been declared with \declaretheorem
% 	\AtEndEnvironment{#2}{%
% 		\xdef\pat@label{\expandafter\expandafter\expandafter
% 			\@fourthoffour\csname thmt@original@#2\endcsname\space\@currentlabel}%
% 		\xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
% 	}%
% 	\else
% 	% the theorem has been declared with \newtheorem
% 	\AtEndEnvironment{#2}{%
% 		\xdef\pat@label{\expandafter\expandafter\expandafter
% 			\@fourthoffour\csname #1\endcsname\space\@currentlabel}%
% 		\xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
% 	}%
% 	\fi
% 	\@namedef{pat@proofof@#2}{#1}%
% }

% % We allocate a block of 1000 token registers; in this way \prooftoks
% % is 1000 and we can access the following registers of the block by
% % \prooftoks+n (0<n<1000); we'll use a dedicated counter for it
% % that is stepped at every proof
% \globtoksblk\prooftoks{1000}
% \newcounter{proofcount}

% % We gather the contents of the proof as argument to \proofatend
% % and then we store
% % "\begin{proof}[Proof of <theoremname> <theoremnumber>]#1\end{proof}"
% % in the next token register of the allocated block
% \NewEnviron{proofatend}{%
% 	\edef\next{%
% 		\noexpand\begin{proof}[\pat@proofof\space\pat@label]%
% 			\unexpanded\expandafter{\BODY}}%
% 		\global\toks\numexpr\prooftoks+\value{proofcount}\relax=\expandafter{\next\end{proof}}
% 	\stepcounter{proofcount}}

% % \printproofs simply loops over the used token registers of the
% % block, freeing their contents
% \def\printproofs{%
% 	\count@=\z@
% 	\loop
% 	\the\toks\numexpr\prooftoks+\count@\relax
% 	\ifnum\count@<\value{proofcount}%
% 	\advance\count@\@ne
% 	\repeat}
% \makeatother

% %% Here starts the example, with two theorem declarations
% %\declaretheorem[style=plain,name=Theorem,qed=$\square$,numberwithin=section]{thm}
% %%\declaretheorem[style=plain,name=Lemma,qed=$\square$,numberlike=thm]{lem}
% %%\newtheorem{thm}{Theorem}
% %\newtheorem{lem}[thm]{Lemma}
% %\fixstatement{thm}
% %\fixstatement[Demonstration of]{lem}

% \fixstatement{lemma}
% \fixstatement{theorem}
% \fixstatement{proposition}
% \fixstatement{corollary}

==> tables/10shot_split1.tex <==
\begin{table}[h!]
\centering
    \caption{10-shot imitation learning results (task success rate).}
    \label{tab:10shot}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c c c c c c}
\hline
Method & Hand Insert & Box Close & Bin Picking & Door Lock & Door Unlock \\
\hline
BC from scratch & $50.8\pm 9.4$ & $55.8 \pm 11.6$ & $60.8 \pm 6.6$ & $52.5 \pm 4.1$ & $98.3 \pm 1.2$  \\
\hline
BC w. pretrained visual encoder & $77.5\pm 6.0$ & $73.3\pm 7.7$ & $80.0\pm 5.4$ & $62.5\pm 2.0$ & $100.0\pm 0.0$ \\
\hline
Ours without BPE & $70.0\pm 5.4$ & $\mathbf{76.8\pm 5.1}$ & $76.5\pm 4.3$ & $91.8\pm 10.0$ & $\mathbf{100.0 \pm 0.0}$ \\
\hline
\rowcolor{gray!25}
Ours with BPE & $\mathbf{84.3 \pm 5.2}$ & $74.0\pm 4.3$ & $\mathbf{81.8\pm 5.2}$ & $\mathbf{92.0\pm 4.0}$ & $\mathbf{100.0\pm 0.0}$ \\
\hline
\end{tabular}
}
\end{table}


==> tables/3shot_split1.tex <==



\begin{table}[h]
\centering
    \caption{3-shot imitation learning results (task success rate). Results are aggregated over 4 random seeds. For the all the method, the agent is finetuned from 50,000 gradient steps, and it is evaluated for 40 episodes every 5000 step. For each seed, we report the best evaluation success rate across all evaluation checkpoints.}
    \label{tab:3shot}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c c c c c c}
\hline
Method & Hand Insert & Box Close & Bin Picking & Door Lock & Door Unlock \\
\hline
BC from scratch & $24.3\pm 1.2$ & $31.7 \pm 14.3$ & $30.0 \pm 4.1$ & $38.3 \pm 7.7$ & $85.0 \pm 5.4$  \\
\hline
BC w. pretrained visual encoder & $42.5\pm 2.0$ & $45.8\pm 9.2$ & $32.5\pm 3.5$ & $42.5\pm 2.0$ & $97.5\pm 3.5$ \\
\hline
\algo~ without BPE & $33.3\pm 2.4$ & $46.8\pm 6.4 $ & $38.8\pm 1.2$ & $61.8\pm 14.5$ & $\mathbf{100.0 \pm 0.0}$ \\
\hline
\rowcolor{gray!25}
\algo & $\mathbf{46.7 \pm 4.2}$ & $\mathbf{51.3\pm 11.6}$ & $\mathbf{42.5\pm 10.2}$ & $\mathbf{65.8\pm 1.2}$ & $\mathbf{100.0\pm 0.0}$ \\
\hline
\end{tabular}
}
\end{table}



==> tables/5shot_split1.tex <==
\begin{table}[h!]
\centering
    \caption{5-shot imitation learning results (task success rate).}
\label{tab:5shot}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c c c c c c}
\hline
Method & Hand Insert & Box Close & Bin Picking & Door Lock & Door Unlock \\
\hline
BC from scratch & $30.8\pm 8.3$ & $35.0 \pm 10.2$ & $45.0 \pm 4.2$ & $45.0 \pm 9.4$ & $87.5 \pm 6.0$  \\
\hline
BC w. pretrained visual encoder & $58.3\pm 9.4$ & $57.5\pm 10.5$ & $44.3\pm 4.3$ & $48.3\pm 6.3$ & $100.0\pm 0.0$ \\
\hline
Ours without BPE & $48.3\pm 6.5$ & $60.8\pm 15.3 $ & $41.8\pm 2.4$ & $67.5\pm 2.8$ & $\mathbf{100.0 \pm 0.0}$ \\
\hline
\rowcolor{gray!25}
Ours with BPE & $\mathbf{65.8 \pm 3.1}$ & $\mathbf{65.0\pm 12.3}$ & $\mathbf{47.5\pm 2.0}$ & $\mathbf{73.3\pm 6.5}$ & $\mathbf{100.0\pm 0.0}$ \\
\hline
\end{tabular}
}
\end{table}

